Exploring Simple and Transferable Recognition-Aware Image Processing

Recent progress in image recognition has stimulated the deployment of vision systems at an unprecedented scale. As a result, visual data are now often consumed not only by humans but also by machines. Existing image processing methods only optimize for better human perception, yet the resulting images may not be accurately recognized by machines. This can be undesirable, e.g., the images can be improperly handled by search engines or recommendation systems. In this work, we examine simple approaches to improve machine recognition of processed images: optimizing the recognition loss directly on the image processing network or through an intermediate input transformation model. Interestingly, the processing model's ability to enhance recognition quality can transfer when evaluated on models of different architectures, recognized categories, tasks and training datasets. This makes the methods applicable even when we do not have the knowledge of future recognition models, e.g., when uploading processed images to the Internet. We conduct experiments on multiple image processing tasks paired with ImageNet classification and PASCAL VOC detection as recognition tasks. With these simple yet effective methods, substantial accuracy gain can be achieved with strong transferability and minimal image quality loss. Through a user study we further show that the accuracy gain can transfer to a black-box cloud model. Finally, we try to explain this transferability phenomenon by demonstrating the similarities of different models' decision boundaries. Code is available at https://github.com/liuzhuang13/Transferable_RA .

==> experiment_res1.tex <==
% \renewcommand{\bb}[1]{\textbf{#1}}
\newcolumntype{C}{>{\centering\arraybackslash}p{1.9em}}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\begin{table*}[ht]
% \begin{subtable}
\caption{Accuracy (\%) on ImageNet classification. R18 means ResNet-18, etc. The five models achieve 69.8, 76.2, 77.4, 74.7, 73.4 on original images. RA processing techniques substantially boost recognition accuracy. }
\mym
\centering
\small
\begin{tabular}{l|CCCCC|CCCCC|CCCCC}
\hline
\multicolumn{1}{c|}{Task} & \multicolumn{5}{c|}{Super-resolution}                & \multicolumn{5}{c|}{Denoising}                       & \multicolumn{5}{c}{JPEG-deblocking}                  \\ \hline
Classification Model      & R18      & R50      & R101     & D121     & V16      & R18      & R50      & R101     & D121     & V16      & R18      & R50      & R101     & D121     & V16      \\ \hline
No Processing             & 46.3     & 50.4     & 55.5     & 51.6     & 42.1     & 46.8     & 55.8     & 61.3     & 59.7     & 46.7     & 43.1     & 47.7     & 55.2     & 49.2     & 43.9     \\
Plain Processing          & 52.6     & 58.8     & 61.9     & 57.7     & 50.2     & 61.9     & 68.0     & 69.1     & 66.4     & 60.9     & 48.2     & 53.8     & 56.0     & 52.9     & 42.4     \\ \hline
RA Processing             & 61.8     & 67.3     & 69.6     & 66.0     & 61.9     & 65.1     & \bb{71.2} & \bb{72.7} & \bb{69.8} & \bb{66.5} & 57.7     & 63.6     & 65.8     & 62.3     & 56.7     \\
RA, Unsupervised        & 61.3     & 66.9     & 69.4     & 65.3     & 61.0     & 61.7     & 68.6     & 70.8     & 67.1     & 63.6     & 53.8     & 60.4     & 63.4     & 59.7     & 53.1     \\ 
RA w/ Transformer         & \bb{63.0} & \bb{68.2} & \bb{70.1} & \bb{66.5} & \bb{63.0} & \bb{65.2} & 70.9     & 72.3     & 69.6     & 65.9     & \bb{59.8} & \bb{65.1} & \bb{66.7} & \bb{63.9} & \bb{58.7} \\ \hline
\end{tabular}
\label{tab:cls}
\end{table*}


